IMO: Greedy Layer-Wise Sparse Representation Learning for Out-of-Distribution Text Classification with Pre-trained Models

Machine learning models have made incredible progress, but they still struggle when applied to examples from unseen domains. This study focuses on a specific problem of domain generalization, where a model is trained on one source domain and tested on multiple target domains that are unseen during training. We propose IMO: Invariant features Masks for Out-of-Distribution text classification, to achieve OOD generalization by learning invariant features. During training, IMO would learn sparse mask layers to remove irrelevant features for prediction, where the remaining features keep invariant. Additionally, IMO has an attention module at the token level to focus on tokens that are useful for prediction. Our comprehensive experiments show that IMO substantially outperforms strong baselines in terms of various evaluation metrics and settings.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/Exp_Tao.tex <==
\subsection{Tasks and Datasets}
We evaluate our method on binary and multi-class classification. We evaluate the performance of the models using accuracy as the metric for binary classification tasks and macro-F1 as the metric for multi-class classification tasks. To assess the statistical significance of our results, we trained the models using five distinct random seeds. 

The binary sentiment analysis datasets include Amazon Review Polarity \cite{zhang2015character}, Yelp Review Polarity \cite{zhang2015character}, IMDB \cite{maas-EtAl:2011:ACL-HLT2011}, TweetEval Sentiment \cite{barbieri-etal-2020-tweeteval} and Yahoo! Answers Sentiment \cite{li-etal-2019-domain}. TweetEval dataset has three categories: positive, negative, and neutral. We remove all neutral instances to align with other datasets. AG News \cite{10.1145/1062745.1062778, 10.1145/1060745.1060764, NIPS2015_250cf8b5} is a collection of news articles for topic classification tasks. AG News contains news titles, and news descriptions, which belong to four topic classes. We train models on title phrases and test models on descriptions, and vice versa. 
SocialDial \cite{zhan2023socialdial} is a Chinese socially-aware dialogue corpus consisting of two parts: synthetic conversation generated by \chatgpt and human-written conversations. Both are annotated with social factors such as location, social distance, and social relation. We train classification models on synthetic conversations and test models on human-written conversations. The statistics of the datasets can be found in Appendix~\ref{apx:experiment_datasets}.

%\textbf{Binary Classification.} The binary sentiment analysis datasets include Amazon Review Polarity \cite{zhang2015character}, Yelp Review Polarity \cite{zhang2015character}, IMDB \cite{maas-EtAl:2011:ACL-HLT2011}, TweetEval Sentiment \cite{barbieri-etal-2020-tweeteval} and Yahoo! Answers Sentiment \cite{li-etal-2019-domain}. TweetEval dataset has three categories: positive, negative, and neutral. We remove all neutral instances to align with other datasets.

%\textbf{Multi-class Classification.} 
%AG News \cite{10.1145/1062745.1062778, 10.1145/1060745.1060764, NIPS2015_250cf8b5} is a collection of news articles for topic classification tasks. AG News contains news titles, and news descriptions, which belong to four topic classes. For the domain generalization task, we train models on title phrases and test models on descriptions, and vice versa. 
%SocialDial \cite{zhan2023socialdial} is a Chinese socially-aware dialogue corpus consisting of two parts: synthetic conversation generated by \chatgpt and human-written conversations. Both are annotated with social factors such as location, social distance, and social relation. We train classification models on synthetic conversations and test models on human-written conversations.


\input{tables/main_result_sentiment_cls}
\input{tables/main_result_multiclass_cls}


\subsection{Benchmark Approaches and Models}
\paragraph{Empirical Risk Minimization.}
As \cite{gulrajani2021in} showed, simple empirical risk minimization (ERM) outperforms many SOTA domain generalization algorithms. So we  finetune \textbf{\bert} \cite{devlin-etal-2019-bert} and encoder of \textbf{\bart} \cite{lewis-etal-2020-bart} using cross-entropy loss as  baselines. For Chinese text classification, we use \textbf{\bert-zh} \cite{devlin-etal-2019-bert}, \textbf{\bart-zh} \cite{shao2021cpt} and \textbf{\chatyuan} \cite{chatyuan}.

\paragraph{Domain Generalization Models.}
\textbf{PADA} \cite{10.1162/tacl_a_00468} is an example-based autoregressive prompt learning algorithm for domain generalization based on the T5 language model \cite{10.5555/3455716.3455856}. Given an input, PADA first generates a prompt and then predicts the label of input concatenated with this prompt.  
\textbf{PDA} \cite{jia-zhang-2022-prompt} is a prompt-based learning algorithm for domain generalization, which applies vocabulary distribution alignment and feature distribution alignment to reduce the gap between different domains.

\paragraph{Large Language Models.}
As \chatgpt shows promising zero-shot ability on various NLP tasks \cite{openai2023gpt4}, we treat \textbf{\chatgpt} (gpt-3.5-turbo) as a baseline. As datasets for the experiments are publicly available, we are uncertain if they are used in \chatgpt's training.  \textbf{\alpaca} \cite{alpaca} is another baseline, which is finetuned from  LLaMA  7B \cite{touvron2023llama} on 52K instruction-following data generated by self-instruct \cite{wang2022selfinstruct}. \textbf{\alpaca-LoRA} is a finetuned \alpaca model using low-rank adaptation \cite{alpaca-lora,hu2022lora}. \textbf{\chatglm-6B} \cite{chatglm_6b} is an open large language model based on General Language Model \cite{du-etal-2022-glm}, optimized for Chinese question-answering and dialogue. All LLMs use few-shot in-context learning. The specific query templates used for the LLMs can be found in Appendix~\ref{apx:training_details}.

\paragraph{Data Augmentation.}
\citet{wiles2022a, gokhale-etal-2022-generalized} find data augmentation benefit domain generalization tasks. Thus, we use three text data augmentation techniques as baselines. \textbf{\eda} \cite{wei-zou-2019-eda} is a widely used text data augmentation technique, which consists of four simple but powerful operations: synonym replacement, random insertion, random swap, and random deletion. \textbf{\uda} \cite{10.5555/3495724.3496249} use back-translation to generate diverse paraphrases while preserving the semantics of the original sentences. \citet{shiri2023paraphrasing}, henceforth referred to as \textbf{\pgb} for brevity, generates syntactically and lexically diversified paraphrases using a fine-tuned BART.
%\footnote{We use \url{https://github.com/425776024/nlpcda} for Chinese data augmentation, which is a Chinese version of \eda.}

\paragraph{Ablation  Models.}
%\nreza{should this description be moved to the abelation section?}
\reza{%Besides baselines, we also apply ablation studies. 
We use abelated version of our method to the backbone models: \bart, T5, and \bert. We denite them as 
%To distinguish these specific implementations, these implementations are referred to as 
\textbf{\ourmethod-\bart}, \textbf{\ourmethod-T5}, and \textbf{\ourmethod-\bert}. To study the contribution of each component in our approach, we conduct experiments where we exclude the mask layers, attention mechanisms, or both. These models are denoted by \textbf{w/o $\vm$}, \textbf{w/o $\va$}, and \textbf{w/o $\va\vm$}, respectively. 
%indicating the removal of mask layers, attention mechanisms,  and both components respectively. 
Furthermore, we employ various sparsification techniques to implement sparse layers, namely,  \textbf{STR} \cite{pmlr-v119-kusupati20a}, \textbf{STE} \cite{bengio2013estimating,LIU2020Dynamic}, and \textbf{Scalar}, where a learnable single scalar is used instead of the threshold vector $\vs$.  Training details can be found in Appendix~\ref{apx:training_details}.
}

\input{tables/main_result_multiclass_socialdial_cls}


\input{tables/ablation_study_sentiment_cls}
\input{tables/ablation_study_multiclass_cls}

\subsection{Domain Generalization Results}
%Tables~\ref{tab:main_result_sentiment_cls}, ~\ref{tab:main_result_multiclass_cls}, ~\ref{tab:main_result_multiclass_socialdial_cls} present our results. We report the accuracy score for binary classification (\ie sentiment analysis) and the macro-F1 score for multi-class classification. 


\paragraph{Binary Classification.} The results are presented in Table~\ref{tab:main_result_sentiment_cls}, where our method using \bart as backbone (\ie \ourmethod-\bart) outperforms all baselines in 7 of 12 settings. In terms of average accuracy, \ourmethod-\bart reaches the highest result, exhibiting average performance gains of 2.63\% than the best baseline (\ie \chatgpt). Interestingly, \chatgpt stands out as the leading model in 3 out of 12 settings. Notably, \alpaca demonstrates a performance level matching with \chatgpt. \alpaca-LoRA also shows relatively good performance across all settings. In comparison, it remains uncertain whether \chatgpt has been trained on the datasets used in this paper. To the best of our knowledge, it is unlikely that \alpaca and \alpaca-LoRA have been trained on these datasets. These observations indicate the strong generalization ability of large language models. Moreover, it is noteworthy that data augmentation methods (\ie \bert-\eda, \bert-\uda, \bert-\pgb) show slightly inferior performance in comparison to the simple fine-tuning of \bert in terms of average accuracy. This suggests that simply back-translating or paraphrasing instances within source domains does not enhance performance on target domains. A plausible explanation could be that augmented data inherently belongs to source domains. Thus, while training on such data might improve performance in source domains, it is unlikely to increase performance in unseen target domains. 

\paragraph{Multi-class Classification.} The results are presented in Table~\ref{tab:main_result_multiclass_cls} and ~\ref{tab:main_result_multiclass_socialdial_cls}. Our method outperforms all baselines in terms of average macro-F1 by 3.22\% and 5.16\% on AG News and SocialDial respectively. Among baselines, \chatgpt exhibits the strongest performance on both datasets and surpasses \alpaca, \alpaca-LoRA, and \chatglm by a large margin. This superior performance shows that current open-source large language models still have a substantial performance gap with \chatgpt when handling difficult tasks.


\subsection{Analysis}
\label{sec:empirical_justification}


\paragraph{Presence of Invariant Representations.} We visualize the masks of the top layer in multiple domains in Fig. \ref{fig:mask_layer_visual_bart} (see Appendix A3). A close inspection shows that there are indeed several features shared across domains. We further compute Cosine similarities between the masks of the top layer trained on different source domains. As shown in Table \ref{tab:mask_vector_cosine_similarity}, the similarities between masks range from 0.68 and 0.85. The token-level sparsity is illustrated by the attention weights visualized in Fig.\ref{fig:attention_weights_yelp} (see Appendix A3) to show the presence of shared key words across domains. 

\paragraph{Impact of Spurious Correlations.}
To study whether our proposed masking mechanism indeed identifies robust features, we conduct experiments where we replace the learned binary masks $\mathbf{q}$ by $\left| 1-\mathbf{q} \right|$. We freeze all parameters except the classification head, then train a model using spurious features identified by $\left| 1-\mathbf{q} \right|$. The results in Table~\ref{tab:study_reverse_mask} show that models using spurious features have an approximate 6\% accuracy reduction in source domains and perform also worse than using all features. In target domains, the corresponding performance decrease using spurious features is significantly higher than both our method and the models using all features.

\input{tables/study_reverse_mask}

\paragraph{Ablation Study.}
We compare top-down greedy search with alternative methods: bottom-up layer-wise search (B2T), simultaneous search (w/o \textbf{sq}), and only applying a mask on the last layer (last). From Table~\ref{tab:main_result_sentiment_cls},~\ref{tab:main_result_multiclass_cls} and ~\ref{tab:main_result_multiclass_socialdial_cls}, we can tell that top-down greedy performs significantly better than the alternative competitors. We conjecture that top-down layer-wise learning serves a regularization method that reduces the risk of loosing crucial features that are well correlated with $Y$ and the corresponding optimization problem is easier to solve than learning all mask layers simultaneously. Representations from higher layers are shown to be more context-specific than lower layer representations~\cite{ethayarajh2019contextual}. In contrast, the bottom up approach may loose key features in lower layers that significantly contribute to higher layer features despite their low correlations to $Y$.

We compare variants of \ourmethod and report the results in Table~\ref{tab:ablation_study_sentiment_cls} and ~\ref{tab:ablation_study_multiclass_cls}.\footnote{See Table ~\ref{tab:ablation_study_multiclass_socialdial_cls} in the Appendix for more results.} Compared with variants that remove both the attention module and mask layers, \ourmethod with the attention module or mask module has a performance improvement in terms of average accuracy or average F1, which suggests the two modules promote performance mutually. Moreover, we replace different backbone models. The experiment results suggest that encoder-decoder pre-trained language models have (\ie \bart, T5) present better performance than encoder-only language models (\ie \bert). 

Additionally, we compare \ourmethod with various sparsity methods to implement mask layers. The experiment results are presented in Table~\ref{tab:ablation_study_sentiment_cls}. STE provides a distinct derivative estimation of the unit step function, exhibiting a marginally lesser impact on our approach. STR, another threshold-based method to implement sparsity in neural networks, results in a performance decline but can achieve higher sparsity in mask layers. Scalar, a variant of our method, substitutes threshold vectors with a single learnable scalar, severely reducing its capacity to achieve sparsity in mask layers. 


\input{tables/different_training_size}

\paragraph{Training Data Size in Source Domains.}
To explore the influence of source domain training data size on performance within target domains, we train models based on \bart with and without our method on the Amazon review dataset with varying sizes of training data (\ie 1k, 10k, 100k, 1M, and 3.6M). The results in Table~\ref{tab:different_training_size} show that our method depends significantly less on training data size, though more training data can improve the performance overall. Notably, 1k training data yields a remarkable decline for the models without using \ourmethod, while the corresponding performance reduction is significantly less by using our method. %These findings imply that a training data size of at least 100k is preferable to ensure the satisfactory performance of our method. Compared to our method, the ablation models lacking the mask and attention mechanisms significantly underperform across all training data sizes. Our method, when trained on only 1k samples, outperforms the ablation models trained on the full dataset.



% \paragraph{Visual Explanation.}
% To intuitively show how the attention module and mask module work in models, we visualize attention weights on tokens and mask vectors in Figure~\ref{fig:attention_weights_yelp} and~\ref{fig:mask_layer_visual_bart}, respectively. We also demonstrate cosine similarities between mask vectors $\vm$ trained on different source domains and Jaccard similarities between binary vectors $\vq$ trained on different source domains on Table~\ref{tab:mask_vector_cosine_similarity} and Table~\ref{tab:binary_vector_Jaccard_similarity}, respectively.

% From Figure~\ref{fig:attention_weights_yelp}, we can find that our model primarily focuses its attention on sentiment-indicative tokens. Notably, positive reviews exhibit high attention weights for tokens like `good,' `great,' and `nice,' indicating their significance. Conversely, negative reviews assign high attention weights to tokens such as `horrible' and `slow,' highlighting their importance in expressing negativity.

% In Figure~\ref{fig:mask_layer_visual_bart}, we visualize mask vectors $\vm$ and binary vectors $\vq$ trained on different source domains across dimensions. It can be observed that certain dimensions are consistently assigned zero (or non-zero) values across different training domains, indicating our mask layers can capture some features that are irrelevant (or invariant) across domains. We quantify invariant features across domains by computing vector similarity. We calculate cosine similarities between different mask vectors $\vm$. The results are shown in Table~\ref{tab:mask_vector_cosine_similarity}. We can find that most mask vector pairs have over $0.75$ similarity, except the Yelp-TweetEval pair, which is probably because of a larger divergence between Yelp and TweetEval domains. Table~\ref{tab:binary_vector_Jaccard_similarity} shows Jaccard similarities between binary vectors $\vq$. Most binary vector pairs have similarities of over $0.5$, except the Yelp-TweetEval pair, with a similarity of $0.45$.





==> sections/intro_tao.tex <==
In the field of natural language processing (NLP), machine learning models have made remarkable advancements \cite{devlin-etal-2019-bert, radford2019language, lewis-etal-2020-bart, NEURIPS2020_1457c0d6, openai2023gpt4, 10.1162/tacl_a_00561}. While these models achieve human-surpassing performance in experimental conditions, researchers have unveiled their vulnerability when confronted with data distribution that differs from the training distribution. This performance gap is caused by the violation of a fundamental assumption in machine learning: training and test data are identically and independently distributed (\ie \textit{i.i.d.} assumption). In real-world scenarios, maintaining the \textit{i.i.d.} assumption is challenging, as domain shifts frequently occur between training and test domains. Therefore, Domain Generalization (DG) has attracted increasing attention from both academic and industrial fields. DG aims to develop models that can generalize effectively to unseen target domains, addressing the challenge of domain shifts.

DG problems can be classified into two categories: multi-source DG and single-source DG. Multi-source DG assumes multiple distinct but relevant domains are available during training, while single-source DG assumes training data is homogeneous. Compared with multi-source DG, single-source DG is more prevalent in real-world scenarios due to the limited availability of multiple source domains. Existing works have made considerable success in addressing multi-source DG through techniques such as data augmentation or prompt learning \cite{10.1007/978-3-030-58545-7_18,9879527,10.1162/tacl_a_00468,jia-zhang-2022-prompt}. However, we argue that existing methods face significant challenges when applied to the single-source DG setting. 

In this paper, we focus on the research topic of single-source DG in the context of text classification. The goal is to develop a model that can generalize to multiple unseen domains using training data from a single domain. It's important to note that all source and target domains share the same label space. 

To address this problem, we propose a novel approach named IMG: \textbf{I}nvariant features \textbf{M}asks for \textbf{G}eneralization. The foundation of our approach is from the Invariance Assumption \cite{10.2307/44682904} which posits that the conditional distribution of the target variable, given the invariant features, will not change across various domains. Inspired by this idea, we propose to apply trainable mask layers to extract invariant features, along with token-level attention modules to capture relevant information at the token level. 

Concretely, we make the following contributions:
\begin{itemize}
    \item We introduce an approach, \ourmethod: \textbf{I}nvariant features \textbf{M}asks for \textbf{G}eneralization, which learns invariant features for consistently predicting target labels across diverse unseen domains. Comprehensive experiment results demonstrate \ourmethod outperforms most strong baselines on multiple text classification tasks under the domain generalization setting.
    \item We develop a theoretical framework that elucidates the relationship between invariant features and causal features. Additionally, we provide an explanation of how our method learns invariant features. 
    \item We verify our model's ability on learning invariant features by visualizing mask layers trained on different domains and computing similarities between these layers. By visually inspecting the mask layers and evaluating their similarities, we provide empirical evidence supporting the claim that our model can capture invariant features.
\end{itemize}
